Second-Order Occlusion-Aware Volumetric Radiance Caching

We present a second-order gradient analysis of light transport in participating media and use this to develop an improved radiance caching algorithm for volumetric light transport. We adaptively sample and interpolate radiance from sparse points in the medium using a second-order Hessian-based error metric to determine when interpolation is appropriate. We derive our metric from each point's incoming light field, computed by using a proxy triangulation-based representation of the radiance reflected by the surrounding medium and geometry. We use this representation to efficiently compute the first- and second-order derivatives of the radiance at the cache points while accounting for occlusion changes. We also propose a self-contained two-dimensional model for light transport in media and use it to validate and analyze our approach, demonstrating that our method outperforms previous radiance caching algorithms both in terms of accurate derivative estimates and final radiance extrapolation. We generalize these findings to practical three-dimensional scenarios, where we show improved results while reducing computation time by up to 30\% compared to previous work.

==> Makefile_latex <==
# make -f Makefile_latex

R = template
STY = *.cls
FIG = images/samplefigure.pdf

pdf: $(R).pdf

$(R).bbl: $(R).bib
	latex $(R)
	bibtex $(R)
	latex $(R)

$(R).ps: *.tex $(STY) $(FIG) $(R).bbl
	latex $(R)
	dvips -Ppdf -G0 -t letter $(R)

$(R).pdf: $(R).ps
	ps2pdf -dPDFSETTINGS=/prepress \
	-dCompatibilityLevel=1.4 \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dMonoImageFilter=/FlateEncode \
	-dDownsampleColorImages=false \
	-dDownsampleGrayImages=false $(R).ps $(R).pdf

clean:
	rm -f $(R).log $(R).aux $(R).bbl $(R).blg $(R).dvi $(R).ps $(R).out


==> macro_last_update.tex <==
% D-Day calculation
\usepackage{datenumber}
\usepackage{calc}

\newcounter{datetoday}
\newcounter{diffyears}
\newcounter{diffmonths}
\newcounter{diffdays}

\newcommand{\difftoday}[3]{%
      \setmydatenumber{datetoday}{\the\year}{\the\month}{\the\day}%
      \setmydatenumber{diffdays}{#1}{#2}{#3}%
      \addtocounter{diffdays}{-\thedatetoday}%
      \ifnum\value{diffdays}>0
        \def\diffbefore{}%
        \def\diffafter{left}%
      \else
        \def\diffbefore{}%
        \def\diffafter{ago}%
        \setcounter{diffdays}{-\value{diffdays}}%
      \fi
      \setcounter{diffyears}{\value{diffdays}/365}%
      \setcounter{diffdays}{\value{diffdays}-365*\value{diffyears}}%
      \setcounter{diffmonths}{\value{diffdays}/30}%
      \setcounter{diffdays}{\value{diffdays}-30*\value{diffmonths}}%
      %
      \diffbefore
      \ifnum\value{diffyears}=0
      \else
        \ifnum\value{diffyears}>1
            \thediffyears\space years,
        \else
            \thediffyears\space year,
        \fi
      \fi
      \ifnum\value{diffmonths}=0
      \else
        \ifnum\value{diffmonths}>1
            \thediffmonths\space months
        \else
            \thediffmonths\space month
        \fi
      \fi
      \ifnum\value{diffdays}=0
      \else
        \ifnum\value{diffdays}>1
            \thediffdays\space days
        \else
            \thediffdays\space day
        \fi
      \fi
      \diffafter
}

==> patches.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Patch for fixing line numbers in paragraphs that contain math environments.
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
	\expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
	\expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
	\renewenvironment{#1}%
	{\linenomath\csname old#1\endcsname}%
	{\csname oldend#1\endcsname\endlinenomath}}% 
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
	\patchAmsMathEnvironmentForLineno{#1}%
	\patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
	\patchBothAmsMathEnvironmentsForLineno{equation}%
	\patchBothAmsMathEnvironmentsForLineno{align}%
	\patchBothAmsMathEnvironmentsForLineno{flalign}%
	\patchBothAmsMathEnvironmentsForLineno{alignat}%
	\patchBothAmsMathEnvironmentsForLineno{gather}%
	\patchBothAmsMathEnvironmentsForLineno{multline}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> src_acks.tex <==
\section*{{ACKNOWLEDGMENTS}}
%We want to thank M.S. Suraj for help with figures. 

==> sup4_errorestimate.tex <==
%!TEX root = sup_main.tex

\section{Second-order error control for media radiance extrapolation}
\label{sup:errorMetricSecondOrder}
The error control in radiance caching is mainly dependent on the error introduced by extrapolation from the radiance cache points. This error is controlled by an error tolerance value $\sErrorTolerance$, and depends on how radiance is extrapolated in the cache neighborhood, as well as on the radiance moments at cache point $\xm$. These in the end give a valid bounding region $\VRegion$ that determines whether a point $\xpr$ is suitable for extrapolation. Jarosz et al.'s~\shortcite{jarosz08radiance} existing radius computation technique is based on local contrast of media radiance, and only relies on first-order derivatives. In practice this leads to cache distributions of points that usually oversample radiance close to surfaces, while undersampling regions far from light sources (see main text, \Fig{crossShadows}).
%

Given the radiance and the first $n$ derivatives at a media point \xm, we can compute the approximated radiance at point $\xpr \in \VRegion$ using a $n\th$-order Taylor expansion as:
%
\begin{align}
\hat{\Rad}_{n}(\xpr) = \sum_{j=0}^n \frac{\Rad^{(j)}(\xm)}{j!} {\left(\Deltaxpr\right)}^j
\label{eq:sup:taylor_expansion}
\end{align}
%
where ${\Deltaxpr = \xpr - \xm}$, and $\Rad^{(j)}(\xm)$ indicates the $j\th$ translational derivative of radiance at \xm.
%
%This approximation introduces an error
%\begin{align}
%\sError_n({\xpr}) &= |\Rad(\xpr) - \hat{\Rad}_{n}(\xpr)| = \Remainder{\xpr}{n},
%\end{align}
%where $\Remainder{\xpr}{n}$ is the remainder of the Taylor expansion of order $n$ \diegoc{we seem to be giving two names to the same thing}. Unfortunately, we cannot compute the exact value of $\sError_n(\xpr)$, since this would require knowing the exact value of the radiance $\Rad(\xpr)$. Moreover, given that we cannot guarantee continuity of $\Rad^{(j)}$ in the closed interval between $\xm$ and $\xpr$, and its immediately higher-order derivative $\Rad^{(j+1)}$ is unknown \diegoc{CHECK: I changed superindices to j, according to the equation}, we cannot compute explicitly the remainder using e.g. its Lagrange or its integral form.
%
This approximation introduces an error
%
\begin{align}
\sError_n({\xpr}) &= |\Rad(\xpr) - \hat{\Rad}_{n}(\xpr)|,
\end{align}
%
which is the remainder of the Taylor expansion of order $n$. Unfortunately, we cannot compute the exact value of $\sError_n(\xpr)$, since this would require knowing the exact value of the radiance $\Rad(\xpr)$. Moreover, given that we cannot guarantee continuity of $\Rad^{(j)}$ in the closed interval between $\xm$ and $\xpr$, and its immediately higher-order derivative $\Rad^{(j+1)}$ is unknown, we cannot compute explicitly this error using e.g. its Lagrange or its integral form.

Instead, we can use our best approximation of the actual radiance ---the $n\th$-order Taylor expansion $\hat{\Rad}_{n}(\xpr)$--- to estimate the error of the $(n-1)\th$-order radiance approximation,
 %
\begin{align}
\sError_{n-1}\approx\estErr_{n-1}({\xpr}) &= |\hat{\Rad}_{n}(\xpr) - \hat{\Rad}_{n-1}(\xpr)| \eqbreak
 &= \left|\frac{\Rad^{(n)}(\xm)}{n!} {\left(\Deltaxpr\right)}^n\right|,
 \label{eq:sup:nthTaylorErrorEstimation}
\end{align}
%
which results in an estimated error proportional to the highest known derivative at \xm. This is equivalent to the Lagrange form of the remainder assuming that ${\Rad}^{(n)}$ is constant in the open interval $(\xm,\xpr)$.
% as $\forall\ym\in(\xm,\xpr)$ then $\Rad_{n}(\ym)=\Rad_{n}(\xm)$ \diegoc{this seemed unnecessary}.
This assumption has been used in previous works truncating the Taylor expansion up to order $n=1$~\cite{jarosz08radiance} and $n=2$~\cite{jarosz12theory,schwarzhaupt12practical}, the latter for surfaces only.

Using this error estimation $\estErr_{n-1}$ we can compute the total (estimated) error introduced by a cache point as the integral over its valid region $\VRegion$ as:
%
\begin{align}
\estErr_{n-1}(\VRegion)
& = \int_\VRegion \estErr_{n-1} (\xpr)\diff\xpr.
\label{eq:sup:estErrRegion}
\end{align}
%
The introduced error is therefore proportional to the size of $\VRegion$; by inverting this integral we can therefore compute the maximum region that satisfies $\estErr_{n-1}(\VRegion) < \sErrorTolerance$.
%
To take into account the sensitivity to contrast of the human visual system, we aim to bound the \textit{relative} error $\estRelError_{n-1}(\VRegion)= \estErr_{n-1}(\VRegion)/\Rad(\xm)$.
%
%While this gives the absolute error bound for radiance, it is important to note that according to the Weber's law humans perceive differences (and therefore error) as a relative measure, and therefore a relative error measurement matches better human perception. Therefore, we would like to bound relative error $\estRelError_{n-1}(\VRegion)= \estErr_{n-1}(\VRegion)/\Rad(\xm)$ rather than the absolute error.

\paragraph*{Truncation to Order 2 for Participating Media}
%
Existing work on radiance caching for participating media estimates relative error using radiance gradients at \xpr.
%in order to modulate cache radius depending on the local contrast ${\left|\GRx \Rad\right|}/{ \Rad}$ of radiance (\Eq{jaroszRadius}).
However, ignoring higher order derivatives creates suboptimal cache distributions that often oversample regions near surfaces and light sources. Moreover, this error formulation does not match the radiance extrapolation based on Taylor expansion of order 1. By computing second-order derivatives of media radiance we improve the estimated relative error as
%introduced by a first-order extrapolation as
%
\begin{align}
\estRelError(\xpr)
& = \frac{\left|\DeltaxprT \HSx \Rad(\x) \Deltaxpr\right|}{2\Rad(\xm)},
\label{eq:sup:error}
\end{align}
%
where $\HSx \Rad$ denotes the radiance Hessian; note that we have removed the expansion order to simplify notation. This approach has been successfully used before to estimate error in \textit{surface} irradiance~\cite{jarosz12theory,schwarzhaupt12practical}.

For $\sDimensions$-D participating media, we can compute the estimated relative error for a first-order expansion as the volume integral on the valid region $\VRegion$ around $\xm = \{x_1 \dots \diff x_\sDimensions\}$ as
\begin{align}
\estRelError(\VRegion)
&= \frac{1}{2}\int_{\VRegion\in\sReals^\sDimensions} \frac{|\DeltaxprT \HSx \Rad(\xm) \Deltaxpr|}{\Rad(\xm)} \diff\xm
\end{align}
%
where the Hessian $\HSx \Rad$ is a $\sDimensions\times\sDimensions$ matrix.
%
The $\sDimensions$ eigenvalues $\lambda_{1}\dots\lambda_{\sDimensions}$ of the Hessian allow us to modulate the radius of the valid region differently along the eigenvectors of radiance, to obtain an anisotropic valid region for each cache point, with an error upper bound
\begin{align}
\estRelError(\VRegion) \leq \idotsint\limits_{\VRegion\in\sReals^\sDimensions} \frac{\sum_{i=1}^\sDimensions |\lambda_{i}| {x_i}^2 }{\Rad(\xm)} \diff{x_1} \dots \diff{x_\sDimensions}
\end{align}
where $x_1\dots x_\sDimensions$ lay in the orthonormal space defined the Hessian eigenvectors ${\{\vvec_{\lambda_1} \dots \vvec_{\lambda_\sDimensions}\}}$. Therefore, the valid region for a cache point in a $\sDimensions$-dimensional space is an hyperellipsoid. By integrating the valid region and inverting the inequality we can compute the maximum space on the Hessian eigenspace, satisfying that the relative error is below the threshold $\sErrorTolerance$, as a set of $\sDimensions$ maximum distances $R^{\lambda_1}\dots R^{\lambda_\sDimensions}$. Similarly, we can define a single maximum distance $R$ by choosing only the maximum absolute eigenvalue $\left|\lambda_{1}\right|$, defining a $\sDimensions$-D hypersphere instead of a $\sDimensions$-D hyperellipse.

For $\sDimensions = 2$, we can parameterize the valid region for a given error threshold $\sErrorTolerance$ as the ellipse with radii $R^{\lambda_i}_{\DD}$:
\begin{align}
R_{\DD}^{\lambda_i}  =\sqrt[4]{\frac{4 \Rad(\xm) \sErrorTolerance}{\pi|\lambda_i|}}.
\label{eq:sup:radiusAniso2D}
\end{align}
%
This formula is analogous to the relative error metric presented by Schwarzhaupt and colleagues~\shortcite{schwarzhaupt12practical}, where radii are computed by projecting surface irradiance Hessian over the surface 2D subspace and obtaining its principal components.

Similarly, for a more practical three-dimensional world ($\sDimensions = 3$), the valid region for a cache point becomes an ellipsoid in 3D, parameterizing its radii $R^{\lambda_i}_{\DDD}$ as a function of the relative error threshold $\sErrorTolerance$ as
\begin{align}
R_{\DDD}^{\lambda_i}  =\sqrt[5]{\frac{15 \Rad(\xm) \sErrorTolerance}{4\pi|\lambda_i|}}.
\label{eq:sup:radiusAniso3D}
\end{align}

Note that this second-order error metric and its derived radius formulae assume perfect known values of radiance and its derivatives at $\xm$. In practice, these are usually computed by Monte Carlo tracing radiance across the scene. This leads to other sources of error of different nature, such as variance inherent to Monte Carlo sampling, or bias due to limitations in the derivatives computation method. In \Secs{inscatDerivatives}{results} we describe and illustrate in more detail these sources of error.

While the presented metric describes error introduced by extrapolation from a single cache point, it is common practice to first pre-populate the cache by tracing (a subset) the pixels of the image, and then perform a so-called \textit{overture} pass that renders the final image. This allows the shading values to be \emph{interpolated} (instead of \emph{extrapolated}) from suitable cache points, increasing reconstruction quality. Due to the nature of the metric, only points that ensure a maximum error $\estRelError$ are used to interpolate radiance at \xpr, and therefore the error of the weighted sum is equally upper-bounded by $\estRelError$.

